Mononizing Binocular Videos

This paper presents the idea ofmono-nizingbinocular videos and a frame-work to effectively realize it. Mono-nize means we purposely convert abinocular video into a regular monocular video with the stereo informationimplicitly encoded in a visual but nearly-imperceptible form. Hence, wecan impartially distribute and show the mononized video as an ordinarymonocular video. Unlike ordinary monocular videos, we can restore from itthe original binocular video and show it on a stereoscopic display. To start,we formulate an encoding-and-decoding framework with the pyramidal de-formable fusion module to exploit long-range correspondences between theleft and right views, a quantization layer to suppress the restoring artifacts,and the compression noise simulation module to resist the compressionnoise introduced by modern video codecs. Our framework is self-supervised,as we articulate our objective function with loss terms defined on the input:a monocular term for creating the mononized video, an invertibility termfor restoring the original video, and a temporal term for frame-to-framecoherence. Further, we conducted extensive experiments to evaluate ourgenerated mononized videos and restored binocular videos for diverse typesof images and 3D movies. Quantitative results on both standard metrics anduser perception studies show the effectiveness of our method.

==> fig_teaser_old.tex <==

%------------------------------------------------------------------------------------------------------
\begin{figure}[!t] 
	\centering
	\includegraphics[width=0.99\linewidth]{Figures/teaser.pdf}
	%\includegraphics[width=0.99\linewidth]{Figures/teaser.png}
%	\includegraphics[width=1\linewidth]{Figures/teaser.png}
	\caption{Given a binocular video, our method produces a mononized video that is no different from an ordinary monocular video. So, we can transmit and display it on conventional monocular-video platforms. Interestingly, if a 3D display is available, we can restore the original binocular video from the mononized video and provide stereo viewing on the video.}
%video service.}
 	\label{fig:key_idea}
\end{figure} 
%------------------------------------------------------------------------------------------------------

